Diverse Community Data for Benchmarking Data Privacy Algorithms

The Collaborative Research Cycle (CRC) is a National Institute of Standards and Technology (NIST) benchmarking program intended to strengthen understanding of tabular data deidentification technologies. Deidentification algorithms are vulnerable to the same bias and privacy issues that impact other data analytics and machine learning applications, and can even amplify those issues by contaminating downstream applications. This paper summarizes four CRC contributions: theoretical work on the relationship between diverse populations and challenges for equitable deidentification; public benchmark data focused on diverse populations and challenging features; a comprehensive open source suite of evaluation metrology for deidentified datasets; and an archive of more than 450 deidentified data samples from a broad range of techniques. The initial set of evaluation results demonstrate the value of these tools for investigations in this field.

==> outline.tex <==
% if you need to pass options to natbib, use, e.g.:
%     \PassOptionsToPackage{numbers, compress}{natbib}
% before loading neurips_2023


% ready for submission
\usepackage{neurips_2023}


% to compile a preprint version, e.g., for submission to arXiv, add add the
% [preprint] option:
%     \usepackage[preprint]{neurips_2023}


% to compile a camera-ready version, add the [final] option, e.g.:
%     \usepackage[final]{neurips_2023}


% to avoid loading the natbib package, add option nonatbib:
%    \usepackage[nonatbib]{neurips_2023}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography

\usepackage{comment}

\usepackage{graphicx}
\usepackage{xcolor}

\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{algorithm} 
\usepackage{algpseudocode}

\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}{Corollary}[theorem]

\algnewcommand\algorithmicforeach{\textbf{for each}}
\algdef{S}[FOR]{ForEach}[1]{\algorithmicforeach\ #1\ \algorithmicdo}
\newcommand{\notimplies}{%
  \mathrel{{\ooalign{\hidewidth$\not\phantom{=}$\hidewidth\cr$\implies$}}}}

\title{Diverse Community Data for Benchmarking Data Privacy Algorithms}

\author{Christine, Aniruddha, Karan, Gary, Dhruv
}

\begin{document}

\maketitle

\begin{abstract}

%Machine learning and data-driven decision making are information intensive operations. Publicly released, deidentified datasets are a key avenue to democratize the benefits of big data while preserving individual privacy. Yet, techniques like anonymization or redaction have known privacy risks. 
%Others, such as differentially private synthetic data, offer privacy guarantees but may lack fidelity compared against original records. High levels of heterogeneity tends to compound these issues. In demographic data, sparsely populated categories carry greater risks to privacy by connecting to more uniquely identifiable people. Data heterogeneity expands the data space, leading to greater sparsity. It is therefore critical that we benchmark privacy-preserving approaches against heterogeneous data.  Here, we present the Diverse Communities Excerpts, tabular data and associated metrology tools. These demographic data, curated from the American Community Survey, are realistic, tractable, and of mixed heterogeneity (diverse). We demonstrate that these data show different rates of dispersal for various demographic categories (e.g., race, sex+disability, etc.). We show that greater variable independence is also correlated with dispersion. These observations motivate the use of diverse data as benchmarks and demonstrate these resources presented here provide a robust platform to benchmark, evaluate, and explore privatizing algorithms. 


The Diverse Communities Data Experts are the core of a NIST program to accelerate research and formal understanding of deidentification technologies. Synthetic data is an ambitious attempt to democratize the benefits of big data. Yet, poorly synthesized datasets may have compromised utility, or worse, lead to wrong conclusions, and can expose private information. Diverse subpopulations, heteregeneous non-ordinal data space, and complex dependencies between features pose intense challenges for synthetic data algorithms. These observations motivate the need for real, diverse, and complex benchmark data. This paper introduces four contributions: new theoretical work on the relationship between diverse population and challenge for equitable deidentification, public benchmark data focused on diverse populations curated from the American Community Survey, a novel suite of evaluation metrology for deidentified datasets, and an archive of evaluation results on a host of deidentification techniques. The initial set of evaluation results demonstrate the suitability of the Excerpts for investigations in this field. 


%The Diverse Communities Data Experts are the core of a NIST program to accelerate research and formal understanding of deidentification technologies. The use of macchine learning, potentially unpredictable, and can have significant negative impact if its done poorly.  It's tricky-- diverse subpopulations, heteregeneous non-ordinal data space, dependencies between features, all of these can cause issues for synthetic data algorithms.  To ensure research in these algorithms serves the needs of real data users and fully addresses real world problems, we need very good benchmark data.  
%In this paper we provide three contributions:  New theoretical work on the relationship between diverse populations and challenges for equitable deidentification (by traditional tecniques and modern synthetic data), a set publicly available benchmark data curated from real world ACS data that focuses on diverse populations and exemplifies as well as other real world complexities for deidentification, and an whole batch of evaluation results on different deidentification and synthetic data stuff showing that this thing does what we say it does. 



\end{abstract}

\section{Introduction}  %Gary and Christine 

Advances in machine learning and vast data collection operations have the potential to transform society and daily life. 
Social media platforms, ordinary government record collection, electronic medical health records systems are just a few examples of rich data repositories that could be used to advance understanding, establish policy, expose fraud and waste, and generally improve lives through data-driven decision making. 
Yet, exposing private information contained in these records risks eroding trust and invites nefarious actors to cause limitless harm.

Deidentification technologies seek to balance the risk of re-identification and data utility. 

To maximize the potential of big data while minimizing harm, we must publish and share data to the greatest extent possible and also limit what can be learned about any single individual stored in the data. 


Deidentification is important in a lot of applications-- releasing gov data for transparency and public use, corporate internal and external use to reduce risk and adhere to regulations.   Deidentification is part of what makes data available for researchers in machine learning.   But if it's not done well, if the deidentified data has bias and artifacts, if it erases diverse subgroups or creates spurious new feature relationships, it can cause all sort of problems for downstream uses. 

There's a wide variety of deidentification approaches out there-- DP, Synthetic Data, SDLC.  All of them have their own behavior patterns when they encounter challenging bits in target data.  Trying to track all of that is the ambitious goal of the NIST CRC project, and the Diverse Data Excerpts are how we're doing it.  They're publicly available and though our focus is on data privacy, they may be useful for other things. 

In this paper we begin by using the concept of dispersal rates to formally discuss the tension between diversity, equity and privacy; this is a key factor in understanding and improving the reliability of deid algorithms in real world conditions, and our data excerpts encourage exploration of it.   

We then discuss the other real world hard bits we've baked into these excerpts.  

And finally, we show how they excerpts used in practice, by using them to compare techniques submitted to the CRC program such as GANs, trees, DP marginal methods, genetic algorithms, traditional privacy, etc on a variety of metrics and visualizations. 

 [[These are distinct from and build on other benchmarking approaches like SDGym?  [[[Better go do a round up of all the big surveys of deid stuff out there-- claire's, tumult's, SDGym, anyone else --- joe near might know the full list.]]] They also build on the NIST challenges. At the end of the paper, we review these in the related works]]. 

\section{Distributional Diversity and the Impact of Dispersal Rates}   %Aniruddha and Christine 

\subsection{Defining Dispersal Rates}

--Definition: Small Cell Count 
--Definitions: Dispersal Rate.  
--sub-definition: Dispersal rates aren't equal for all subpopulations 
--Picture that shows impact on the data quality, evidence from the data that this exists and how it arises, impact on cell counts, impact on performance of privacy. 

\subsection{Formal Analysis of Distributional Diversity} 

Plain english outline of the math.   
The notation definitions
The math. 

\subsection{Distributional Diversity in the Diverse Community Excerpts}

Plain english saying that the above isn't an impossibility theorem, it's only a challenging thing.  Different techniques handle it differently, as you'll see in the third section-- some handle it quite well.   But the diverse data do exemplify this challenge. 
Demonstration of this-- should see it be more diverse in the national data than MA and TX. 

\section{Introducing the Diverse Community Excerpts}   %Christine 

\subsection{Geographies}
-Three data sets, what and why (full geography list in appendix?  maps?  link to postcards?)

\subsection{Features Selection}

-demographic
-disability
-etc
-etc

\subsection{Challenges and Opportunities}

we've got
-complex demographic correlations, diversity complexity 
-deterministic feature relationships
-weighting
-high cardinality
-categorical features, numerical and a mix.   
-features with holes in the distribution 
--?

You can use this to: 
-look at equity
-check reidentification
-consider weights
-look at smoothness... ?

\section{Demonstration of the Diverse Community Excerpts as Benchmarking Tools}  %Dhruv and Christine 

A sentence on the CRC program and the breadth of approaches submitted and metrics run.  

An outline of the types of techniques we're showing [GAN, etc-- check Dhruv's list]. 

Some things to look out for. 
--privacy/utility trade-off, not exactly
--equitable performance vs biased utility
--added noise intentional and unintentional, random or shaped
--artifacts and inconsistencies
--unknowns

\subsection{Preserving Diverse Relationships between Education and Income}
Definition of the regression metric. 

\subsection{Propensity, Principle Component Analysis, and Artifacts}
Definition of the propensity metric and PCA visualization.

\subsection{Overall Privacy and Utility}
Definition of unique exact match metric and k-marginal utility score.

\section{Related Works}  %Gary
%Gary

\section{Conclusions}  %Gary
Gary's patented paragraph on the importance of doing this well for king and country, and how there's this benchmark data (combined with the metric suite) will help researchers in the future understand and address many things we don't have a grasp on future, and how we think it's important to make these tools as widely available as possible. 







  
  %(0) What is synthetic data/why?  Deidentified data and why? (note the ML connection, ML in verbose mode) 

  %(1) We're introducing diverse commnity benchmark data and associated new metrics to spport research understanding the behavior of synthetic data algorithms on diverse communities 

  %(2) This is important because models and privacy in general struggle with diverse data distributions, causing equity and bias issues.  We have theoretical work on the interaction between demographic heteregeneous feature dependencies, data sparsity, and utliity disparity for deidentified data.  [ small cell count bad, disperal rate bad, heteregeneous data leads to uneven dispersal rate, diversity leads to heteregeneous data, we need benchmarks for privacy (and possibly ML in general) that focus on diverse communities to learn how different algorithms respond/behave when encountering these challenges in modeling human data. 

  %(3) Here's some data for that (PUMA and features chosen especially for that). And here's a batch of algorithms performing weirdly on it, as promised.
 
  %(3 cont'd)  We define our data and its properties, and demonstrate some of the results of the CRC showing many synthesis techniques using this data (and metrics from the program). All these tools are publicly availalbe.  

  % Christine's notes on item 3: 
  % --------------------------------
  % Explain features (demographic, house, etc, like the readme for the data) 
  % --- including their tricky bits. 
  %
  % probably group symthesizers into SDLC, classical DM, Neural, DP-marginal 
  % Show synthesizer performance on regression metric for different categories of 
  % synthesizers. (got numbers for slope and intercept) 
  % Show propensity metric for everyone, in a table. 
  % Consider adding an evaluation task where it's using the synthetic data to 
  % predict if a row has more than $50K income (maybe make it a report metric
  % use a decision tree)-- trains on the synthetic data, predicts on the target



\section{Related Work}

\section{Conclusion, Future Work}


\section*{References}

\small
[1] Alexander, J.A.\ \& Mozer, M.C.\ (1995) Template-based algorithms for
connectionist rule extraction. In G.\ Tesauro, D.S.\ Touretzky and T.K.\ Leen
(eds.), {\it Advances in Neural Information Processing Systems 7},
pp.\ 609--616. Cambridge, MA: MIT Press.

\end{document}

